Quantifying Local and Global Fidelity of Nonlinear Embeddings

Dimension reduction rests on a claim: t-SNE and UMAP preserve local structure, PCA global structure. Our DLP curve is the share of each point's k nearest neighbors a map keeps. Corrected for chance, it gives L at k=10 and G over 30 to 50% of the data, local and global fidelity. At the midpoint the curve is provably a rank correlation of distances. The LG reversal test decides, with a stated error rate, which of two maps is local and which global. On twelve datasets of up to 1.38 million points, G agrees with established global scores at 0.84 and 0.93, and the area under R_NX at 0.22 and 0.30. The entity fidelity E, read at each point's entity size, predicts which entities a map loses beyond L and G where entity sizes differ. In an agent memory of one million passages, t-SNE and PCA cross at 150,000 passages (p=2.6e-5).

==> tab_LG_rows.tex <==
PCA & .71/\textbf{.94} & .33/\textbf{.71} & .23/\textbf{.70} & .12/\textbf{.46} & .04/\textbf{.34} & .41/.24 & .45/.29 & .10/.53 \\
KPCA & .52/.78 & .30/.59 & .16/.52 & .12/.29 & .04/.33 & .41/.26 & .52/.52 & .01/.01 \\
LLE & .37/.55 & .24/.44 & .13/.46 & .18/.29 & .11/.16 & .63/.60 & .55/.55 & .33/.57 \\
Isomap & .67/.86 & .34/.70 & .23/\textbf{.70} & .19/.42 & .06/\textbf{.34} & \textbf{.88}/\textbf{.98} & \textbf{.80}/\textbf{.90} & .22/\textbf{.60} \\
t-SNE, PCA init & \textbf{.79}/.81 & \textbf{.59}/.68 & .46/.56 & \textbf{.57}/.34 & \textbf{.46}/.29 & .85/.84 & .78/.85 & \textbf{.51}/.55 \\
t-SNE, random init$^\dagger$ & .78/.82 & \textbf{.59}/.68 & \textbf{.47}/.57 & \textbf{.57}/.33 & \textbf{.46}/.28 & .85/.82 & .78/.82 & \textbf{.51}/.51 \\
UMAP$^\dagger$ & .71/.79 & .56/.66 & .41/.57 & .47/.28 & .32/.21 & .77/.85 & .72/.85 & .42/.42 \\
PHATE$^\dagger$ & .54/.79 & .33/.66 & .29/.55 & .32/.30 & .18/.26 & .56/.73 & .56/.75 & .32/.25 \\
PaCMAP$^\dagger$ & .67/.81 & .53/.60 & .36/.54 & .41/.31 & .26/.17 & .79/.66 & .74/.81 & .40/.52 \\
TriMAP$^\dagger$ & .66/.80 & .53/.63 & .37/.57 & .42/.34 & .26/.19 & .72/.57 & .69/.71 & .40/.57 \\

==> tab_embodied_rows.tex <==
raw & 180 & .420 & [.33, .50] & .298 & .005 & 2.51 & -- & 1,358 & 0.155 & 0.093 \\
\addlinespace
PCA(3) & 3 & .319 & [.24, .39] & .312 & .035 & 0.16 & 0.18 & 88 & 0.874 & 0.859 \\
NPCA(3) & 3 & .305 & [.23, .38] & .290 & .037 & 0.16 & 0.50 & 88 & 0.863 & 0.844 \\
PCA(5) & 5 & .414 & [.33, .50] & .359 & .024 & 0.19 & 0.18 & 102 & 0.864 & 0.864 \\
NPCA(5) & 5 & .400 & [.31, .47] & .354 & .029 & 0.20 & 0.61 & 110 & 0.813 & 0.812 \\
PCA(10) & 10 & .466 & [.37, .55] & .368 & .016 & 0.29 & 0.18 & 158 & 0.673 & 0.650 \\
NPCA(10) & 10 & .470 & [.38, .56] & .364 & .022 & 0.26 & 0.92 & 143 & 0.721 & 0.704 \\
PCA(20) & 20 & .465 & [.37, .55] & .349 & .012 & 0.43 & 0.18 & 232 & 0.519 & 0.475 \\
NPCA(20) & 20 & .474 & [.39, .56] & .353 & .017 & 0.42 & 2.95 & 228 & 0.531 & 0.486 \\
\addlinespace
Isomap(3) & 3 & .265 & [.19, .34] & .228 & .010 & 52 & 228 & 28,248 & 0.018 & 0.005 \\
LLE(3) & 3 & .237 & [.17, .31] & .197 & .013 & 2.15 & 47 & 1,210 & 0.140 & 0.103 \\
UMAP(3)$^\dagger$ & 3 & .291 & [.21, .37] & .308 & .018 & 1.89 & 128 & 1,149 & 0.159 & 0.114 \\
PHATE(3)$^\dagger$ & 3 & .304 & [.21, .38] & .232 & .018 & 123 & 217 & 66,513 & 0.010 & 0.002 \\
t-SNE(3)$^\dagger$ & 3 & .408 & [.32, .49] & .330 & .027 & 1,197 & 683 & 647,171 & 0.003 & $<$.001 \\
\addlinespace
Isomap(10) & 10 & .365 & [.27, .45] & .303 & $-$.007 & 51 & 590 & 27,949 & 0.020 & 0.005 \\
UMAP(10) & 10 & .311 & [.22, .39] & .310 & .024 & 2.10 & 178 & 1,311 & 0.150 & 0.102 \\
t-SNE(2) & 2 & .395 & [.31, .48] & .321 & .021 & 737 & 347 & 398,159 & 0.003 & $<$.001 \\


==> tab_large_LG_rows.tex <==
Pathology-100K & 0.012 & 0.008 & 0.436 & 0.331 & \textbf{0.458} & 0.233 & 0.205 & \textbf{0.597} & 0.461 & 0.442 & 0.456 & 0.442 & 0.290 & 0.494 \\
SEA-AD (single cell) & 0.000 & 0.000 & 0.082 & 0.048 & \textbf{0.117} & 0.018 & 0.014 & 0.286 & 0.285 & 0.243 & 0.232 & 0.243 & 0.340 & \textbf{0.417} \\
Instacart (supply chain) & 0.001 & 0.001 & 0.102 & 0.057 & \textbf{0.123} & 0.009 & 0.004 & 0.213 & 0.211 & 0.236 & 0.254 & 0.236 & 0.221 & \textbf{0.268} \\
MS MARCO (agent memory) & 0.000 & 0.000 & 0.253 & 0.200 & \textbf{0.309} & 0.065 & 0.030 & \textbf{0.283} & 0.188 & 0.222 & 0.227 & 0.222 & 0.153 & 0.211 \\
\midrule
MNIST & 0.007 & 0.008 & 0.377 & 0.289 & \textbf{0.390} & 0.153 & 0.103 & \textbf{0.301} & 0.266 & 0.187 & 0.205 & 0.187 & 0.106 & 0.117 \\
CIFAR-10 & 0.002 & 0.002 & 0.199 & 0.125 & \textbf{0.200} & 0.037 & 0.023 & 0.327 & 0.303 & 0.297 & 0.324 & 0.297 & \textbf{0.328} & 0.326 \\
Fashion-MNIST & 0.013 & 0.013 & 0.326 & 0.232 & \textbf{0.336} & 0.113 & 0.082 & \textbf{0.743} & 0.701 & 0.471 & 0.492 & 0.472 & 0.456 & 0.451 \\
Speech Commands & 0.010 & 0.009 & 0.300 & 0.224 & \textbf{0.301} & 0.052 & 0.032 & \textbf{0.668} & 0.655 & 0.544 & 0.565 & 0.544 & 0.591 & 0.597 \\
Renal-Cortex & 0.012 & 0.012 & 0.315 & 0.202 & \textbf{0.327} & 0.141 & 0.120 & 0.385 & \textbf{0.387} & 0.327 & 0.325 & 0.328 & 0.283 & 0.311 \\
Brain-Cortex & 0.006 & 0.006 & 0.334 & 0.215 & \textbf{0.346} & 0.140 & 0.116 & 0.328 & 0.322 & 0.317 & 0.317 & 0.317 & 0.356 & \textbf{0.413} \\
Covertype & 0.036 & 0.036 & 0.624 & 0.455 & \textbf{0.638} & 0.389 & 0.298 & 0.302 & 0.258 & 0.197 & 0.187 & 0.197 & 0.184 & \textbf{0.328} \\
AG News & 0.005 & 0.004 & 0.341 & 0.276 & \textbf{0.341} & 0.133 & 0.085 & \textbf{0.414} & 0.351 & 0.329 & 0.344 & 0.330 & 0.327 & 0.329 \\


==> tab_large_data_rows.tex <==
Pathology-100K & Pathology & 100,000 & 768 & Phikon \\
SEA-AD (single cell) & Single cell & 1,378,211 & 50 & 50 PCs \\
Instacart (supply chain) & Supply chain & 195,827 & 2,000 & purchases \\
MS MARCO (agent memory) & Agent memory & 1,000,000 & 768 & BGE-base \\
\midrule
MNIST & Vision & 70,000 & 784 & pixels \\
CIFAR-10 & Vision & 60,000 & 512 & ResNet-18 \\
Fashion-MNIST & Vision & 70,000 & 784 & pixels \\
Speech Commands & Audio & 59,387 & 768 & wav2vec 2.0 \\
Renal-Cortex & Single cell & 50,027 & 50 & 50 PCs \\
Brain-Cortex & Single cell & 50,212 & 50 & 50 PCs \\
Covertype & Remote sensing & 59,999 & 54 & attributes \\
AG News & Text & 60,000 & 768 & BERT \\


==> tab_own_rows.tex <==
Pathology-100K & 0.012/0.597 & 0.008/0.461 & 0.436/0.442 & 0.458/0.442 & $+0.022$ & $-0.0004$ \\
SEA-AD & 0.000/0.286 & 0.000/0.285 & 0.082/0.243 & 0.117/0.243 & $+0.036$ & $-0.0000$ \\
Instacart & 0.001/0.213 & 0.001/0.211 & 0.102/0.236 & 0.123/0.236 & $+0.021$ & $-0.0001$ \\
MS MARCO & 0.000/0.283 & 0.000/0.188 & 0.253/0.222 & 0.309/0.222 & $+0.056$ & $-0.0000$ \\
\midrule
MNIST & 0.007/0.301 & 0.008/0.266 & 0.377/0.187 & 0.390/0.187 & $+0.013$ & $+0.0004$ \\
CIFAR-10 & 0.002/0.327 & 0.002/0.303 & 0.199/0.297 & 0.200/0.297 & $+0.001$ & $+0.0001$ \\
Fashion-MNIST & 0.013/0.743 & 0.013/0.701 & 0.326/0.471 & 0.336/0.472 & $+0.010$ & $+0.0002$ \\
Speech Commands & 0.010/0.668 & 0.009/0.655 & 0.300/0.544 & 0.301/0.544 & $+0.000$ & $-0.0001$ \\
Renal-Cortex & 0.012/0.385 & 0.012/0.387 & 0.315/0.327 & 0.327/0.328 & $+0.013$ & $+0.0003$ \\
Brain-Cortex & 0.006/0.328 & 0.006/0.322 & 0.334/0.317 & 0.346/0.317 & $+0.011$ & $-0.0003$ \\
Covertype & 0.036/0.302 & 0.036/0.258 & 0.624/0.197 & 0.638/0.197 & $+0.014$ & $-0.0003$ \\
AG News & 0.005/0.414 & 0.004/0.351 & 0.341/0.329 & 0.341/0.330 & $+0.000$ & $+0.0005$ \\


==> tab_pairs_rows.tex <==
Pathology-100K & $\mathbf{1.8\times10^{-4}}$ & 0.3 & $\mathbf{1.6\times10^{-3}}$ & 0.6 & $\mathbf{1.5\times10^{-3}}$ & 0.4 & $0.28$ & 33.8 & $0.28$ & 33.7 & $0.129$ & $\mathbf{2.6\times10^{-4}}$ \\
SEA-AD & $0.063$ & 1.0 & $\mathbf{3.5\times10^{-5}}$ & 0.9 & $\mathbf{3.5\times10^{-5}}$ & 0.9 & $0.17$ & 34.5 & $0.17$ & 34.5 & $0.002$ & $\mathbf{5.3\times10^{-3}}$ \\
Instacart & $\mathbf{8.1\times10^{-3}}$ & 4.5 & $\mathbf{7.6\times10^{-6}}$ & 8.4 & $\mathbf{7.4\times10^{-6}}$ & 8.4 & $0.81$ & 99.3 & $0.81$ & 99.3 & $0.001$ & $0.48$ \\
MS MARCO & $\mathbf{8.1\times10^{-4}}$ & 0.7 & $0.94$ & 1.1 & $0.94$ & 1.1 & $0.96$ & 64.6 & $0.96$ & 64.6 & $0.092$ & $\mathbf{1.4\times10^{-8}}$ \\
\midrule
MNIST & $0.20$ & 2.2 & $1.00$ & 1.5 & $1.00$ & 1.4 & $0.080$ & 25.2 & $0.081$ & 25.2 & $0.035$ & $\mathbf{1.6\times10^{-3}}$ \\
CIFAR-10 & $0.47$ & 6.9 & $\mathbf{0.012}$ & 5.9 & $\mathbf{0.011}$ & 5.7 & $0.53$ & 39.8 & $0.53$ & 39.9 & $0.028$ & $\mathbf{0.013}$ \\
Fashion-MNIST & $0.89$ & 2.2 & $0.85$ & 1.5 & $0.85$ & 1.4 & $\mathbf{4.3\times10^{-7}}$ & 11.0 & $\mathbf{4.3\times10^{-7}}$ & 11.0 & $0.042$ & $\mathbf{1.4\times10^{-3}}$ \\
Speech Commands & $\mathbf{0.018}$ & 7.6 & $\mathbf{4.6\times10^{-9}}$ & 3.6 & $\mathbf{4.3\times10^{-9}}$ & 3.6 & $\mathbf{3.6\times10^{-5}}$ & 18.2 & $\mathbf{3.5\times10^{-5}}$ & 18.2 & $0.012$ & $\mathbf{3.1\times10^{-3}}$ \\
Renal-Cortex & $0.23$ & 2.3 & $0.79$ & 1.4 & $0.79$ & 1.1 & $0.14$ & 30.1 & $0.14$ & 30.2 & $-0.002$ & $0.94$ \\
Brain-Cortex & $\mathbf{0.049}$ & 1.4 & $\mathbf{1.3\times10^{-3}}$ & 1.3 & $\mathbf{1.2\times10^{-3}}$ & 1.0 & $0.51$ & 40.6 & $0.51$ & 40.6 & $0.007$ & $0.16$ \\
Covertype & $\mathbf{1.5\times10^{-3}}$ & 0.6 & $\mathbf{6.3\times10^{-3}}$ & 1.1 & $\mathbf{6.1\times10^{-3}}$ & 0.7 & $\mathbf{0.013}$ & 22.9 & $\mathbf{0.012}$ & 22.7 & $0.043$ & $\mathbf{7.3\times10^{-3}}$ \\
AG News & $0.45$ & 2.5 & $0.59$ & 1.8 & $0.60$ & 1.7 & $\mathbf{0.04999}$ & 31.8 & $0.053$ & 31.9 & $0.066$ & $\mathbf{3.3\times10^{-6}}$ \\


==> tab_sens_rows.tex <==
$G$, $0.3\le k/n\le0.5$ (default) & 1.000 & 1.00 & 1.00 & 0.84 & 0.93 \\
$G$, $0.2\le k/n\le0.5$ & 0.982 & 0.83 & 0.43 & 0.80 & 0.91 \\
$G$, $0.4\le k/n\le0.5$ & 0.979 & 0.89 & 0.52 & 0.91 & 0.97 \\
Midpoint $\nu_{k^\star}$ & 0.957 & 0.79 & 0.24 & 0.94 & 0.98 \\
Middle band, $0.1\le k/n\le0.2$ & 0.752 & 0.15 & $-$0.81 & 0.57 & 0.70 \\


==> tab_sim_rows.tex <==
Pathology-100K & +0.155 & 0.0029 & 0.0205 & 0.0019 & 0.00 & 0.00 & 0.06 & 0.14 & 1.00 & 0.101 (0.003) \\
SEA-AD & +0.043 & 0.0061 & 0.0441 & 0.0030 & 0.00 & 0.00 & 0.14 & 0.18 & 0.00 & 0.344 (0.008) \\
Instacart & -0.023 & 0.0025 & 0.0096 & 0.0018 & 0.00 & 0.00 & 0.14 & 0.08 & 0.00 & 0.986 (0.014) \\
MS MARCO & +0.061 & 0.0037 & 0.0125 & 0.0015 & 0.00 & 0.00 & 0.14 & 0.22 & 1.00 & 0.145 (0.006) \\
\midrule
MNIST & +0.114 & 0.0048 & 0.0378 & 0.0031 & 0.00 & 0.00 & 0.10 & 0.28 & 1.00 & 0.190 (0.004) \\
CIFAR-10 & +0.030 & 0.0041 & 0.0235 & 0.0019 & 0.00 & 0.00 & 0.14 & 0.28 & 0.00 & 0.307 (0.008) \\
Fashion-MNIST & +0.272 & 0.0044 & 0.0278 & 0.0022 & 0.00 & 0.00 & 0.06 & 0.02 & 1.00 & 0.092 (0.002) \\
Speech Commands & +0.124 & 0.0031 & 0.0197 & 0.0019 & 0.00 & 0.00 & 0.08 & 0.24 & 1.00 & 0.163 (0.004) \\
Renal-Cortex & +0.057 & 0.0049 & 0.0617 & 0.0029 & 0.00 & 0.00 & 0.20 & 0.14 & 0.00 & 0.302 (0.008) \\
Brain-Cortex & +0.011 & 0.0079 & 0.0370 & 0.0025 & 0.00 & 0.00 & 0.08 & 0.10 & 0.00 & 0.401 (0.006) \\
Covertype & +0.105 & 0.0043 & 0.0234 & 0.0018 & 0.00 & 0.00 & 0.10 & 0.26 & 1.00 & 0.179 (0.003) \\
AG News & +0.085 & 0.0036 & 0.0146 & 0.0013 & 0.00 & 0.00 & 0.06 & 0.34 & 1.00 & 0.180 (0.004) \\


==> tab_sweep_rows.tex <==
t-SNE, perplexity & 5 & 0.363 & 0.189 & 0.050 & 1,986 \\
 & 15 & 0.379 & 0.220 & 0.036 & 2,692 \\
 & 30 & 0.370 & 0.218 & 0.038 & 3,424 \\
 & 50 & 0.354 & 0.244 & 0.004 & 4,246 \\
 & 100 & 0.315 & 0.234 & 0.007 & 7,164 \\
 & 200 & 0.259 & 0.255 & 0.011 & 11,480 \\
 & 500 & 0.180 & 0.269 & 0.003 & 21,359 \\
\addlinespace
UMAP, \texttt{n\_neighbors} & 5 & 0.151 & 0.218 & 0.010 & 953 \\
 & 15 & 0.110 & 0.206 & 0.001 & 1,055 \\
 & 50 & 0.087 & 0.206 & 0.002 & 1,629 \\
 & 100 & 0.078 & 0.214 & 0.005 & 2,289 \\
 & 200 & 0.071 & 0.223 & 0.001 & 3,385 \\
 & 500 & 0.063 & 0.220 & 0.013 & 5,556 \\
\addlinespace
t-SNE, exaggeration & 1 & 0.370 & 0.218 & 0.038 & 3,617 \\
 & 2 & 0.158 & 0.212 & 0.031 & 2,928 \\
 & 4 & 0.100 & 0.205 & 0.022 & 3,003 \\
 & 8 & 0.077 & 0.209 & 0.019 & 3,085 \\
 & 16 & 0.059 & 0.232 & 0.002 & 3,065 \\
 & 32 & 0.045 & 0.229 & 0.001 & 2,971 \\
\addlinespace
PCA($q$) + t-SNE, $q$ & 2 & 0.008 & 0.146 & 0.128 & 3,445 \\
 & 5 & 0.084 & 0.311 & 0.001 & 3,238 \\
 & 10 & 0.201 & 0.269 & 0.028 & 3,009 \\
 & 30 & 0.326 & 0.206 & 0.032 & 2,864 \\
 & 50 & 0.353 & 0.218 & 0.036 & 2,800 \\


==> tab_validation_rows.tex <==
$L=\nu_{10}$ (exact) & $-$0.18 & $-$0.10 \\
Middle band, $0.1\le k/n\le0.2$ & 0.57 & 0.70 \\
Area under $R_{NX}$ & 0.22 & 0.30 \\
$G$, $0.2\le k/n\le0.5$ & 0.80 & 0.91 \\
$G$, $0.3\le k/n\le0.5$ & \textbf{0.84} & \textbf{0.93} \\
$G$, $0.4\le k/n\le0.5$ & 0.91 & 0.97 \\
Midpoint $\nu_{k^\star}$ & 0.94 & 0.98 \\

